Experimental Design for Linear Functionals in Reproducing Kernel Hilbert Spaces

Optimal experimental design seeks to determine the most informative allocation of experiments to infer an unknown statistical quantity. In this work, we investigate the optimal design of experiments for {\em estimation of linear functionals in reproducing kernel Hilbert spaces (RKHSs)}. This problem has been extensively studied in the linear regression setting under an estimability condition, which allows estimating parameters without bias. We generalize this framework to RKHSs, and allow for the linear functional to be only approximately inferred, i.e., with a fixed bias. This scenario captures many important modern applications, such as estimation of gradient maps, integrals, and solutions to differential equations. We provide algorithms for constructing bias-aware designs for linear functionals. We derive non-asymptotic confidence sets for fixed and adaptive designs under sub-Gaussian noise, enabling us to certify estimation with bounded error with high probability.

==> arxiv/applications.tex <==
%\begin{figure}[h]
%	\includegraphics[width=0.45\textwidth]{pic/grads.png}
%	\caption{Gradient estimation. The upper plot shows the total error of $\nabla f(x)$ we can certify with high probability as a function of the step-size $h$ for a finite difference design. The minima of these errors exactly correspond to  step-sizes derived from the bias-variance trade-off we proposed for the interpolation estimator. With increasing $T$, noise can be reduced more, and hence bias of the design needs to decrease accordingly, hence the decrease in the step size (e.g.,
%~red$\to$green). The value of $\nu^2$ is always for the optimal E-design.}
%	\label{fig:grads}
%\end{figure}

\begin{figure*}
	\begin{subfigure}{0.33\textwidth}
		\includegraphics[width=\textwidth]{pic/pharmaco.png}
		\caption{Pharmacokinetics}
		\label{fig:pharma}
	\end{subfigure}
	\begin{subfigure}{0.33\textwidth}
%			\begin{subfigure}{0.49\textwidth}
%\includegraphics[width=\textwidth]{pic/contamination.png}				\caption{Statistical contamination }
	\includegraphics[width=\textwidth]{pic/grads.png}
		\caption{Gradient estimation}
		\label{fig:grads}
	\end{subfigure}
	\begin{subfigure}{0.33\textwidth}
		\includegraphics[width=\textwidth]{pic/control.png}
		\caption{Controller stability}
		\label{fig:control}
	\end{subfigure}

%	\begin{subfigure}{0.66\textwidth}
%	\includegraphics[width=\textwidth]{pic/sub-space.png}
%	\caption{}
%	\label{fig:cnvx}
%\end{subfigure}
    \vspace{-0.1cm}
	\caption{Experiments: \textbf{a) } \emph{Pharmacokinetics}. We compare the equally spaced design (black) with the optimized design (yellow). The optimized design mimics the classical pharmacokinetics approach of spreading the initial measurements more densely after the initial dose \citep{Gabrielsson1995}. For us, this rule elegantly emerges from first principles. In general, these trajectories follow a decaying trajectory as the examples in light purple. The uncertainty in $c_b$ is due to the unknown dynamics $\gamma$ is depicted in shaded region. \textbf{ b)} \emph{Gradient estimation}. The upper plot shows the total error of $\nabla f(x)$ we can certify with high probability as a function of the step-size $h$ for a finite difference design. The minima of these errors exactly correspond to  step-sizes derived from the bias-variance trade-off we proposed for the interpolation estimator. With increasing $T$, noise can be reduced more, and hence bias of the design needs to decrease accordingly, hence the decrease in the step size (e.g.,~red$\to$green). \textbf{c)} \emph{Stability:} We report the upper bound on the Lyapunov function in the whole operating domain, as a function of data points. The color coding (explained in the text) represents different data acquisition algorithms while dashed lines correspond to the confidence sets from prior work. Our confidence sets (solid) provide a tighter upper bound as a function of the number of data points, and allows faster termination, which happens when the upper bound is zero. }
	\label{fig:applications}
	\vspace{-0.5cm}
\end{figure*}
\vspace{-0.25cm}
\section{Applications} \label{sec:example} \looseness -1
We now discuss concrete applications that benefit from our contributions. Details of the experiments, and further applications, e.g., in statistical contamination, can be found in Appendices \ref{app:examples} and \ref{app:experiments}. 
\vspace{-0.2cm}
\subsection{Gradient maps} \looseness -1 \label{sec:derivatives}
Gradients of any order are linear operators. We can express the gradient at $x$ as dimension-wise evaluation of the following operator
$ \nabla_x (\Phi(x)^\top\theta) = (\nabla_x \Phi(x))^\top\theta =: \bC \theta. $
Clearly, estimability is nearly always impossible, since any evaluation infinitesimally away from $x$ will be insufficient to eliminate bias. Thus our estimates will invariably be biased for any function with infinite Taylor expansion. Yet, while estimating the gradient from evaluations very close to the original $x$ leads to low bias, it at the same time increases the variance, since the difference in the functional value between the two point evaluations is very small compared to the noise magnitude. Given a finite budget or desired accuracy, the best we can do is to find the best design with optimal bias-variance trade-off given the kernel $\kappa$, budget $T$, and noise variance $\sigma$. We consider a class of parametrized finite difference designs $\{\Phi(x \pm he_i)\}$, where $h$ is the stepsize and $e_i$ are unit vectors. In Fig.~\ref{fig:grads}, we plot the total error with high probability with the budget $T$ as a function of the step-size $h$. Notice that the lowest error occurs exactly when the variance of observations scaled with the confidence parameter is equal to the relative $\nu$ (two lines cross).
\vspace{-0.2cm}
%\vspace{-0.2cm}
\subsection{Learning linear ODE solutions and their parameters}\label{sec:example:odes}
\looseness -1 A solution to a linear ordinary differential equation (ODE) $u$ satisfies  $\frac{d}{dt} u(t) = \bM u(t) + s(t)$, where $\bM$ is a linear operator and $s(t)$ is the non-homogeneous term. Assume that the solution to the equation $u(t) =\Phi(t)^\top u$ is a member of a Hilbert space $\mH_\kappa$, then $\bT u :=  \left(\frac{d}{dt} - \bM(t) \right) \Phi(t)^\top u = s(t)$ for $ t \in [t_0, t_1].$ Hence, the differential equation becomes a \emph{linear constraint} for estimating  $u$ from samples. In fact, due to differential equations being fully specified by initial conditions, the only unknowns are due to initial conditions. To reveal the linear functional here, one needs to consider the solution to the differential equation, which can be written as $u = \bT^\dagger s(t) + \bC^\top v $, where $v \in \mH_\kappa \setminus \Span(\bT)$ belongs to the null space of $\bT$. In this case, we span it with rows of $\bC$. Consequently, the unknown element $v$ can be found as $\bC (u-\bT^\dagger s)$. Thus, what needs to be estimated from samples, is the linear projection $\bC u$, since $\bC\bT^\dagger s$ is known a priori. In Appendix \ref{app:experiments}, we discuss implementation and calculation of the operator $\bC$ on a discretized domain. 

%Also note that, $\bZ$ itself induces a Hilbert space $\mH_z$ containing the solutions $u$ \citep{Gonzalez2014}. However, as we will see, for robust designs it is sometimes convenient to pick a larger Hilbert space $\mH_\kappa$ s.t.
%$\mH_z \subset \mH_\kappa$ and then apply the differential equation constraint. 

\vspace{-0.1cm}
\paragraph{Robust Design} \looseness -1 As a specific example, consider an example of a pharmacokinetic model capturing the concentration of a medication in blood and stomach via differential equations: $(d/dt) c_s = -a c_s$ and $(d/dt) c_b = b c_s - d c_b~\text{for} ~ t \in [t_0, t_1]$, where $c_s$ and $c_b$ are the concentration in stomach and blood respectively. The goal of this analysis is to infer $\gamma = (a,b,d)$ from the measurements of the blood concentration levels with fixed, but perhaps noisy, initial conditions \citep{Gabrielsson1995}. To apply the above procedure, we need a fixed differential operator $\bT_\gamma$ to define the operator $\bC_\gamma$. However, $\gamma$ is itself unknown. Instead, we can give a generally plausible set of $\gamma \in \Gamma$, initial conditions of concentration in blood $c_b(0) = 0$, and norm constraints on the initial stomach concentration $(c_s(0)-c_{\text{dose}})^2\leq \lambda^{-1}$ (prior $\mV_0$) in order to apply our framework. We use the squared exponential kernel to embed trajectories and consider robust $A$-optimal design (as in Sec.~\ref{sec:designs}) by maximizing the worst case metric $\inf_{\gamma \in \Gamma}\Tr((\bC_\gamma\bV_\lambda^{-1}\bC_\gamma^\top)^{-1} )$ with the regularized estimator. This way, the design is appropriate for any $\gamma$. After estimating the trajectory, we can use the estimated trajectories  (given $\gamma$) to optimize for $\gamma$ via the maximum likelihood. Fig.~\ref{fig:odeint} presents the concentrations $c_b$ and $c_s$ with their estimates and uncertainties due to the unknown $\gamma$. We show the equally spaced  (black) and optimized designs (yellow). The more accurately we can infer the trajectory, the more accurately we can estimate $\gamma$, which we quantitatively show  in Appendix \ref{app:examples} in Fig.~\ref{fig:pharm}, where we decrease the MSE of estimating $\gamma$ by a factor of $10$ in comparison to equally spaced design.

% Note that $\bZ$ itself induces a Hilbert space $\mH_z$ containing the solutions $u$ \citep{Gonzalez2014}, and we could use that directly. However, as we will see, for robust designs it is convenient to pick a larger Hilbert space $\mH_\kappa$ s.t.
%~$\mH_z \subset \mH_\kappa$. 
\vspace{-0.2cm}
\subsection{Sequential Design: Certifying Lyapunov Stability}
Consider a non-linear system with $x \in \mR^d$ such that $ \frac{d}{dt}x(t) = f(x(t),t) + u(x(t),t) =
\bA \Phi(x(t),t) + u(x(t),t)$, where the rows of $\bA_i \in \mH_\kappa$ for $i\in [d]$ model the system dynamics and $\Phi(x(t),t)$ are known evaluation functionals of $\mH_\kappa$. We assume that the control laws $u(x(t),t)$ can be written as $u(x(t),t) = \bB \Phi(x(t),t)$. We want to understand whether a given a control law $\bB$ stabilizes the above system. A common approach is to create an estimate $\hat{\bA}$ of $\bA$ from data samples of trajectories, and use the controller $\bB = \hat{\bA} - \bP$, where $\bP$ is often a simple reverting law with a known gain. With this choice of $u$, the system can be written as
$\frac{d}{dt}x(t) = (\bA - \hat{\bA} -\bP)\Phi(x(t),t) = (\tilde{\bA}-\bP)\Phi(x(t),t)$
where the $\tilde{\bA}$ is uncertain. We can certify the stability of the resulting system using a \emph{known} quadratic Lyapunov function, e.g., $V(x,t) = (x(t)-x_\text{ref}(t))^\top \bSigma (x(t)-x_\text{ref}(t))$. Classical stability theory dictates that if the total derivative of $V$, 
\begin{equation}\label{eq:lyapunov-function}
	dV/dt= (x(t)-x_{\text{ref}}(t))^\top \bSigma (\tilde{\bA}-\bP) \phi(x(t),t) +{\partial V}/{\partial t},
\end{equation}
is negative for all $x(t) \in \mO$ then we can guarantee stability in the operating region of $x \in \mO$ \citep{Khalil2002}. The above condition defines a linear operator $\bC_x = (x-x_{\text{ref}})^\top \bSigma\cdot\phi(x)$ operating on the unknown $\tilde{\bA}$ for each $x \in \mO$. The linearity is best seen with vectorization as $\theta = \operatorname{vec}(\bA)$, using the shorthand $z(t) = x(t) - x_{\text{ref}}(t)$,
$ z^\top \bSigma \bA \phi(x) = \operatorname{vec}(\bSigma z\phi(x)^\top)^\top \operatorname{vec}(\bA) = \bC_x \theta.  $
The operator is parametrized by $x$, $\bC_x$ for each $x \in \mO$. Even for continuous domains $x \in \mO$, $\bC_x$ usually has low-rank structure, which can be calculated and depends on the size $\mO$ and the size $\mH_\kappa$. If the rank of the operator is small (e.g., the operating space is small) then we can certify negativity of Eq.~\eqref{eq:lyapunov-function} faster than learning the whole $\bA$. In other words, we reduce uncertainty only where we need to as in the seminal work of \citet{Berkenkamp2016}. We can sequentially query data points from $x$ and check whether $\bC_{x}\theta \leq 0$ for all $x$. 

\looseness-1 Consider a two dimensional nonlinear system from \citet{Lederer2020},
\[ \frac{dx}{dt} = x + \frac{1}{1+\exp(-2x_1)} \begin{pmatrix}1 \\ -1 \end{pmatrix} + 0.5  \begin{pmatrix}\sin(\pi x_2) \\ \cos(\pi x_1) \end{pmatrix} + u. \]
The reverting controller is $\bP\Phi(x(t),t) = -K (x - x_{\text{ref}}(t))+(d/dt)x_{\text{ref}}$, where the reference trajectory corresponds to a circle $x_{\text{ref}}(t) = ( \sin(t), \cos(t))$. The Lyapunov function is $V = (x(t) - x_{\text{ref}}(t))^\top(x(t) - x_{\text{ref}}(t))$. We assume that we can set the system to an initial condition $x(0)$ and observe a noisy observations of the state $y(0+\Delta)$ at rapid sampling times $\Delta$. From these, we create a derivative oracle, $(d/dt) x(t) \approx (x(t+\Delta) - x(t))/\Delta$, a common approach in nonlinear data-driven control \citep{Umlauft2018}. We use this example to showcase our adaptive confidence sets. We follow an adaptive stopping rule, where we query new data points if negativity cannot be certified. Due to this adaptive stopping rule, the data is adaptively collected. We compare our confidence sets (solid) with the classical confidence sets of \citet{Abbasi-Yadkori2011} (dashed) and report upper bounds on the supremum over $x \in \mO$ of Eq.~\eqref{eq:lyapunov-function} in Fig.~\ref{fig:control}. The operating region is a ``tube'' around the circular reference trajectory $x_{\text{ref}}(t)$. We see that our confidence sets shrink much faster than the classical confidence sets, since we can eliminate redundant information by projecting onto $\bC$. Fig.~\ref{fig:control} compares random sampling of datapoints from the whole domain (random) and the operating region (random-ref) and sampling according to uncertainty in the dynamics in the whole domain (unc) and within the tube around the reference trajectory (unc-ref). As expected, focused exploration methods work much better. However, and more importantly, the tightness of our confidence sets enable much quicker stability certification (termination). Note that the classical confidence sets may even {\em grow} in the cases where redundant information for estimation of $\bC$ is inserted into the estimation, e.g., with random sampling.
